A New Semi-supervised Learning Benchmark for Classifying View and Diagnosing Aortic Stenosis from Echocardiograms

Semi-supervised image classification has shown substantial progress in learning from limited labeled data, but recent advances remain largely untested for clinical applications. Motivated by the urgent need to improve timely diagnosis of life-threatening heart conditions, especially aortic stenosis, we develop a benchmark dataset to assess semi-supervised approaches to two tasks relevant to cardiac ultrasound (echocardiogram) interpretation: view classification and disease severity classification. We find that a state-of-the-art method called MixMatch achieves promising gains in heldout accuracy on both tasks, learning from a large volume of truly unlabeled images as well as a labeled set collected at great expense to achieve better performance than is possible with the labeled set alone. We further pursue patient-level diagnosis prediction, which requires aggregating across hundreds of images of diverse view types, most of which are irrelevant, to make a coherent prediction. The best patient-level performance is achieved by new methods that prioritize diagnosis predictions from images that are predicted to be clinically-relevant views and transfer knowledge from the view task to the diagnosis task. We hope our released Tufts Medical Echocardiogram Dataset and evaluation framework inspire further improvements in multi-task semi-supervised learning for clinical applications.

==> evaluation.tex <==

% THIS SECTION CUT! Relevant content repurposed into results.tex

% \paragraph{Performance metrics.} Throughout this paper, we consider several task-appropriate performance metrics.

%Throughout this paper, for the 3-way view and 3-way diagnosis tasks, we consider \emph{balanced accuracy} as our primary performance metric of interest. This is important because standard accuracy numbers do not adequately reflect performance on tasks with \emph{imbalance}, as our tasks have. For example, on our view classification test set, the ``Other'' category is far more common, representing over 80\% of all images. Trivally guessing ``Other'' for every image would thus reach over 80\% accuracy, but only 33.3\% balanced accuracy.

% Later, for patient-level diagnosis, we also consider FPR at TPR 99\%. 

%% Other 4559-5027 = 4800 = 0.84
%% PLAX   624-646  =  640 = 0.11
%% PSAX   172-212  =  200 = 0.37



==> fig_SevereAS_NoAS_patient_sample.tex <==
% \newcommand{\BA}{0.3}
% \setlength{\tabcolsep}{0.1cm}
% \begin{figure}
% \begin{tabular}{c c c c}
%     PLAX  & PSAX & OTHER 
%     \\
%     \includegraphics[width=\BA\textwidth]{figures/SevereAS_11112007_PLAX1.pdf}
%     &
%     \includegraphics[width=\BA\textwidth]{figures/SevereAS_11112007_PSAX1.pdf}
%     &
%     \includegraphics[width=\BA\textwidth]{figures/SevereAS_11112007_Other1.pdf}
%     &
    
%     \\
    
%     \includegraphics[width=\BA\textwidth]{figures/SevereAS_11112007_PLAX2.pdf}
%     &
%     \includegraphics[width=\BA\textwidth]{figures/SevereAS_11112007_PSAX2.pdf}
%     &
%     \includegraphics[width=\BA\textwidth]{figures/SevereAS_11112007_Other2.pdf}
%     &
   
%      \\
     
%      \includegraphics[width=\BA\textwidth]{figures/SevereAS_11112007_PLAX3.pdf}
%     &
%     \includegraphics[width=\BA\textwidth]{figures/SevereAS_11112007_PSAX3.pdf}
%     &
%     \includegraphics[width=\BA\textwidth]{figures/SevereAS_11112007_Other3.pdf}
%     &
  
%     \end{tabular}	
%     \caption{Examples of images from a patient with Severe AS in our dataset. \emph{From left to right:} Three examples of parasternal long axis (PLAX) view, three examples of parasternal short axis (PSAX) view, and three examples of other kinds of view in our ``Other'' class. }
%     \label{fig:PatientSevereAS}
% \end{figure}


% \newcommand{\BB}{0.3}
% \setlength{\tabcolsep}{0.1cm}
% \begin{figure}
% \begin{tabular}{c c c c}
%     PLAX  & PSAX & OTHER 
%     \\
%     \includegraphics[width=\BB\textwidth]{figures/NoAS_1996889_PLAX1.pdf}
%     &
%     \includegraphics[width=\BB\textwidth]{figures/NoAS_1996889_PSAX1.pdf}
%     &
%     \includegraphics[width=\BB\textwidth]{figures/NoAS_1996889_Other1.pdf}
%     &
    
%     \\
    
%     \includegraphics[width=\BB\textwidth]{figures/NoAS_1996889_PLAX2.pdf}
%     &
%     \includegraphics[width=\BB\textwidth]{figures/NoAS_1996889_PSAX2.pdf}
%     &
%     \includegraphics[width=\BB\textwidth]{figures/NoAS_1996889_Other2.pdf}
%     &
   
%      \\
     
%      \includegraphics[width=\BB\textwidth]{figures/NoAS_1996889_PLAX3.pdf}
%     &
%     \includegraphics[width=\BB\textwidth]{figures/NoAS_1996889_PSAX3.pdf}
%     &
%     \includegraphics[width=\BB\textwidth]{figures/NoAS_1996889_Other3.pdf}
%     &
  
%     \end{tabular}	
%     \caption{Examples of images from a patient with No AS in our dataset. \emph{From left to right:} Three examples of parasternal long axis (PLAX) view, three examples of parasternal short axis (PSAX) view, and three examples of other kinds of view in our ``Other'' class. }
%     \label{fig:PatientNoAS}
% \end{figure}
